Scaling 3D Reasoning with LMMs to Large Robot Mission Environments Using Datagraphs

This paper addresses the challenge of scaling Large Multimodal Models (LMMs) to expansive 3D environments. Solving this open problem is especially relevant for robot deployment in many first-responder scenarios, such as search-and-rescue missions that cover vast spaces. The use of LMMs in these settings is currently hampered by the strict context windows that limit the LMM's input size. We therefore introduce a novel approach that utilizes a datagraph structure, which allows the LMM to iteratively query smaller sections of a large environment. Using the datagraph in conjunction with graph traversal algorithms, we can prioritize the most relevant locations to the query, thereby improving the scalability of 3D scene language tasks. We illustrate the datagraph using 3D scenes, but these can be easily substituted by other dense modalities that represent the environment, such as pointclouds or Gaussian splats. We demonstrate the potential to use the datagraph for two 3D scene language task use cases, in a search-and-rescue mission example.

==> src/archive/datagraphdiagram.tex <==
\tikzstyle{wp} = [circle, minimum width=1.5cm, minimum height=1.5cm, text centered, draw=black, fill=red!30, font=\footnotesize]
\tikzstyle{wo} = [circle, minimum width=1.5cm, minimum height=1.5cm, text centered, draw=black, fill=blue!50, font=\footnotesize]
\tikzstyle{ft} = [circle, minimum width=1.5cm, minimum height=1.5cm, text centered, draw=black, fill=green!30, font=\footnotesize]
\tikzstyle{agent} = [circle, minimum width=1.5cm, minimum height=1.5cm, text centered, draw=black, fill=yellow!50, font=\footnotesize]

\tikzstyle{goto} = [<->, >=stealth, color=red, line width=5pt]
\tikzstyle{behavior} = [->, >=stealth, color=blue, line width=5pt]
\tikzstyle{explore} = [->, >=stealth, color=red, line width=5pt]

% \tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]
% \tikzstyle{arrow} = [thick,->,>=stealth]
% \tikzstyle{myBlock} = [rectangle, minimum width=2.5cm, minimum height=1.5cm, text centered, draw=black, fill=green!30, font=\footnotesize]


% from the intro
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=1cm,text centered, draw=black, fill=white!30, font=\small]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=orange!30, font=\small]

\newcommand{\gotoBehavior}{\behavior_\text{goTo}}


\begin{figure}[t]
% \begin{figure}[h]
    \centering
    \resizebox{0.40\textwidth}{!}{
    \begin{tikzpicture}[node distance=4cm, align=center]
        \node (wp1) [wp] {\Large $\node_1$};
        \node (wp2) [wp, above of=wp1] {\Large $\node_2$};
        \node (wp3) [wp, right of=wp2] {\Large $\node_3$};
        \node (wp4) [wp, above of=wp3] {\Large $\node_4$};
        \node (ft1) [wo, left of=wp2] {\Large $\object_1$ \\ \\ \Large (frontier)};
        \node (wo1) [wo, below right of=wp3] {\Large $\object_2$\\ \\\Large (chemical\\ \Large container)};
        \node (wo2) [wo, right of=wp4] {\Large $\object_3$\\ \\ \Large (door)};
        
        \draw [goto] (wp1) -- (wp2) node[midway, left] {\Large $\gotoBehavior$};
        \draw [goto] (wp2) -- (wp3) node[midway, above] {\Large $\gotoBehavior$};
        \draw [goto] (wp3) -- (wp4) node[midway, left] {\Large $\gotoBehavior$};
        \draw [behavior] (wp3) -- (wo1) node[midway, above right] {\Large $\behavior_\text{requestTeleop}$};
        \draw [behavior] (wp4) -- (wo2) node[midway, above] {\Large $\behavior_\text{openDoor}$};
        \draw [behavior] (wp2) -- (ft1) node[midway, above] {\Large $\gotoBehavior$};
        \node (agent1) [agent, left of=wp2, xshift=3.2cm, yshift=-0.8cm] {\large robot};
        
        
        \draw [->] (-4,-0.5) -- ++(0.5,0) node[right]{\footnotesize\textit{x}};
        \draw [->] (-4,-0.5) -- ++(0,0.5) node[above]{\footnotesize\textit{y}};
    \end{tikzpicture}
    }\Large 
    \caption{todo}
    \label{fig:datagraph-diagram}
\end{figure}

==> src/archive/related_work.tex <==
% \subsection{Related Work}
% There have been various methods to address the scaling problem for 3D reasoning. 
% In this section, these methods are discussed based on their application to either 2D or 3D models.

% \paragraph{Resolution curse for 2D vision language tasks}
% The resolution curse for 2D tasks is often solved using \emph{tiling} approaches.
% The input image is subsampled into several tiles of lower resolution. 
% Afterwards, the tiles are processed sequentially by the model, thereby avoiding the resolution curse.
% However, creation of the tiles is often done in a naive way, using uniformly distributed tiles \cite{}. Advanced methods such as learning based/attention-based tiling selectors have been proposed \cite{}. Still, a trade-off between redundant overlap and missed detections remains \cite{}. Similarly, the relevant context of the objects (such as adjacent objects) may be lost \cite{}. Finally, it is an open question how far to reduce the resolution of the tiles \cite{}.
% All approaches address the same tile overlapment trade-off.
% When tiles overlap, detections can be duplicated between tiles, leading to the need for deduplication techniques.
% While without overlapping tiles, large objects that might not be detected at all, as both tiles do not hold enough pixels for detection at their boundaries.
% Similarly, the context relevant for the objects (such as adjacent objects) may be lost.


% \paragraph{Resolution curse for 3D scene language tasks}
% The resolution curse also exists for 3D scene. Most LMMs suffer from performance degradation when the input size increases \cite{}. 
% The main reason is ... [cite].
% This limits the usability of these models for real-world applications.
% Furthermore, there are only limited 3D scenes available to facilitate research into large 3D scenes \cite{jia_sceneverse_2024}.
% A visualisation is given in \cref{fig:sceneVerseScenes}.
% It only contains data points at the scale of a floor of a building with up to 5 rooms.
% \cite{chen_leveraging_2023} shows limited performance in performing room classification in small environments.


% LMMs for 3D scenes \cite{} predominately operate on pointclouds, while Gaussian splats \cite{} have also been used.
% \textcite{jia_sceneverse_2024} is the largest available dataset for training LMMs for 3D tasks.
% A visualisation is given in \cref{fig:sceneVerseScenes}.
% It only contains data points at the scale of a floor of a building with up to 5 rooms.
% \cite{chen_leveraging_2023} shows limited performance in performing room classification in small environments.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{resource/scene verse scenes.jpg}
%     \caption{Overview of the largest 3D scene training dataset SceneVerse \cite{jia_sceneverse_2024}. 
%     %contains only medium sized scenes. Floors of buildings with up to 5 rooms. This is not enough for robot deployments in expansive areas of operation, say kilometre scale.
%     }
%     \label{fig:sceneVerseScenes}
% \end{figure}
% % %



% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{resource/3d scene graph.png}
%     \caption{3D scene graphs \cite{rosinol_3d_2020} constitute an alternative approach to environment representation in robotics.}
%     \label{fig:3DsceneGraph}
% \end{figure}

% \paragraph{3D scene graphs as intermediate representation}
% A widely adopted alternative methodology involves the real-time condensation of the environment into a 3D scene graph during the mapping process \cite{armeni_3d_2019, rosinol_3d_2020}, subsequently utilizing this compressed representation for reasoning tasks \cite{rana_sayplan_2023}. This proactive approach is comparable to performing work in advance, rather than retrospectively on demand.

% This method can trade off between memory usage and computational load. 
% The principal advantage of the online 3D scene graph approach is that it compresses information into a manageable representation while retaining most of the data required for mission tasks. 
% However, a notable drawback is the potential loss of critical information during this compression process. 
% The context in which objects are situated is often crucial; for instance, in a first-responder scenario, the distinction between a person lying on the ground and a person sitting in a chair is significant.
% Our proposed datagraph with LMM-based approach could determine whether individuals are in danger by preserving contextual details, whereas the 3D scene graph might discard this essential context.



==> src/archive/results.tex <==
\section{Results}

\begin{itemize}
    \item baseline candidates:
    \begin{itemize}
        \item brute force: search over all images in area. eg. search over all frames of videos stream... guess thats how gpt-4o currently works so relevant benchmark.
    \end{itemize}
    \item comparison of brute force search over all images vs spatially aware search for object retrieval task.
    \item Show that this method finds the closest object instance, and not just any instance.
    \item Plan: take a video in the basement of TNO and sprinkle some interesting objects there.
    \item locker door encountered, mission is to find the key. and you just remembered it is connected to a XXX keyfob.
    \item or matching the numbers on a door with the numbers on a keyfob.
\end{itemize}
